Brief Note: Asynchronous Verifiable Secret Sharing with Optimal Resilience and Linear Amortized Overhead

In this work we present hbAVSS, the Honey Badger of Asynchronous Verifiable Secret Sharing (AVSS) protocols - an AVSS protocol that guarantees linear amortized communication overhead even in the worst case. The best prior work can achieve linear overhead only at a suboptimal resilience level (t < n/4) or by relying on optimism (falling back to quadratic overhead in case of network asynchrony or Byzantine faults). Our protocol therefore closes this gap, showing that linear communication overhead is possible without these compromises. The main idea behind our protocol is what we call the encrypt-and-disperse paradigm: by first applying ordinary public key encryption to the secret shares, we can make use of highly efficient (but not confidentiality preserving) information dispersal primitives. We prove our protocol is secure under a static computationally bounded Byzantine adversary model.

==> avid.tex <==
\subsection{Asynchronous Verifiable Information Dispersal.}
\label{rp2p}
To achieve a linear communication overhead in our AVSS scheme, we also require an efficient and reliable asynchronous messaging
Maybe it should go in the protocol section} protocol. Specifically, we need a bandwidth-efficient protocol that guarantees eventual delivery under an honest dealer and which allows a recipient to prove that a specific message was the same one sent by the dealer in the protocol. 

\begin{definition} (Asynchronous Verifiable Information Dispersal (AVID))
Consider a dealer $D$ and $N > 3t$ parties, where we assume an adversary may corrupt up to $t$ of the parties and possibly the dealer. A Reliable Messaging protocol will achieve the following properties:
\todo{Since these properties essentially mirror those for RBC, lets make them more consistent with RBC}
  \begin{itemize}
      \item \emph{(Liveness)} If the dealer is honest, the recipient will receive a message.
      \item \emph{(Validity)} If the dealer sends $v$, and the recipient receives $v'$, then $v=v'$.
      \item \emph{(Non-repudiability)} Upon receiving $v$ from $D$, a recipient can prove that $v$ is exactly the message sent by $D$. \todo{This "prove" quality should be stated more precisely. We will also need to provide a proof that the RP2P protocol satisfies all these properties }
  \end{itemize}
\label{def:rp2p}
\end{definition}
\todo{Split into properties of two phases}
Our ReliablePointToPoint protocol is shown in Figure \ref{alg:avid}.

\begin{theorem}
RP2P is a reliable messaging protocol
\end{theorem}

\begin{figure}[t]
\begin{boxedminipage}{\columnwidth}
  {\centering \textbf{Algorithm $\msf{AVID}(D,R)$ (with Dealer $D$ and Receiver $R$)} \\}
{\bf Dealer Phase }
  { \hline }
As dealer $D$:
\begin{itemize}
\item upon input$(v)$:
  \begin{itemize}
  \item[] let $\{s_j\}_{j\in[N]}$ be the blocks of an $(N-2f,N)$-erasure coding scheme applied to $v$
  \item[] let $h$ be a Merkle tree root computed over $\{s_j\}$
  \item[] distribute $h$ via $\msf{ReliableBroadcast}(h)$
  \item[] send $\mtt{VAL}(b_j, s_j)$ to each party $\P_j$, where $b_j$ is the $j^{th}$ Merkle tree branch
  \end{itemize}
\end{itemize}
As party $\P_i$:
\begin{itemize}
\item upon receiving $\mtt{VAL}(b_i, s_i)$ from $D$,
  \begin{itemize}
  \item[] send $\mtt{ECHO}(b_i,s_i)$ to $R$
  \item[] check that $b_i$ is a valid Merkle branch for root $h$ and leaf $s_i$ and if so, multicast $\mtt{OK}$
  \end{itemize}
\item upon receiving $\mtt{REVEAL}(\{{b_j}, {s_j}\}_{j\in[f+1]})$ from $R$ ,
  \begin{itemize}
  \item[] verify correctness of the branches and leaves against h
  \item[] recalculate the Merkle root as $h'$.
  \item[] wait until $\mtt{OK}$ has been received from $2f+1$ parties
  \item[] If $h \neq h'$, output $\bot$
  \item[] otherwise, decode and output $v$
  \end{itemize}
\end{itemize}
As party $R$:
\begin{itemize}
\item upon receiving $\mtt{ECHO}(b_j,s_j)$ from party $\P_j$, 
  \begin{itemize}
  \item[] check that $b_j$ is a valid Merkle branch for root $h$ and leaf $s_j$, and otherwise discard
  \end{itemize}
\item upon receiving valid $\mtt{ECHO}(\cdot,\cdot)$ messages from $f+1$ distinct parties,
  \begin{itemize}
  \item[] interpolate $\{s_j\}_{j\in[N]}$ from the $f+1$ leaves 
  \item[] recompute Merkle root $h'$ and if $h' \neq h$ then $\mtt{ReliableBroadcast}(\mtt{REVEAL},\{{b_j}, {s_j}\}_{j\in[f+1]})$, where $(b_j, s_j)$ are branch and leaf combinations that verify against $h$
  \item[] otherwise, decode and output $v$
  \end{itemize}
\item if it is later necessary to prove that $v$ was dealt by $D$,
  \begin{itemize}
    \item[] $\mtt{ReliableBroadcast}(\mtt{REVEAL},\{{b_j}, {s_j}\}_{j\in[f+1]})$, where $(b_j, s_j)$ is a valid branch and leaf combination 
  \end{itemize}
\end{itemize}
\end{boxedminipage}
\caption{Reliable Point To Point messaging algorithm.}
\label{alg:rp2p}
\end{figure}



==> batch.tex <==
\section{Batch AVSS}

In many real world applications, a one-off AVSS may not be sufficient. For example, a sender may wish to send a message that is larger than the finite field, which is likely no bigger than a few hundred bits. A message may be significantly larger and there may even be many of them. We therefore believe that optimizations to AVSS protocols to allow for efficient batch secret sharing are incredibly relevant to a practical implementation. We present cost-saving modifications to our protocols in the batch setting in the following subsections.

\subsection{Reduction of Integrity Check Costs}
The first modification required for the batched version our schemes is very straightforward. The dealer still creates polynomials, commitments, witnesses and shares for each secret to be shared, but now sends them all at once. For example, there is still one instance of ReliableBroadcast, which now sends commitments (and shares and witnesses for hbAVSS-lite) to all of the polynomials along with an ephemeral key. There are also still N instances of ReliablePointToPoint in hbAVSS, which now includes witnesses and shares for all secrets in the batch.

The primary savings achieved here is that since the number of invocations of ReliableBroadcast and ReliablePointToPoint remains the same, the number of Merkle trees that need to be built over erasure-coded data is constant with respect to the batch size. With a sufficiently large batch, the bandwidth cost of this integrity check per-secret approaches zero and the protocols achieve their appropriate linear bandwidth overheads. 

\subsection{More Efficient Dealer Implication}
In hbAVSS, implication requires that a recipient produce the payload it received from the dealer in order to prove that is was malformed. In the case of a Batch AVSS, this would require sending every item in the batch to every peer. This is not optimal and instead it should be sufficient to show that at least one item was malformed to prove a dealer's malfeasance. 

To accomplish this...

\subsection{Cost Improvements}
Todo

\begin{figure*}
  \vspace{10pt}
\begin{boxedminipage}{\columnwidth}
  {\centering \textbf{Algorithm $\msf{hbAVSS}(D)$ (for dealer $D$)} \\}
  {\bf Setup:}
\begin{itemize}
\item Each party $P_i$ is associated with a public key $PK_i$, and knows their own secret key $SK_i$ and public generator $g$, such that $PK_i = g^{SK_i}$
\item Setup the polynomial commitment scheme $SP \leftarrow \msf{Setup}(1^\lambda)$
\end{itemize}
{\bf As dealer $D$:} \\
On input $\{s_1,...,s_{t+1}\}$:
\begin{itemize}
\item[] {\it // Secret share encoding}
\item Generate a random degree-$(t,t)$ bivariate polynomial $\phi(\cdot,\cdot)$ so that $\phi(0,k) = s_k$ and $\phi(i,k)$ is $\P_i$'s share of $s_k$
  \vspace{5pt}
\item[] {\it // Broadcast polynomial commitments}
\item For $k \in [t+1]$: $C_k,\msf{aux}_k \leftarrow \msf{PolyCommit}(SP, \phi(\cdot,k) )$
\item $\msf{ReliableBroadcast}( \{ C_k\}_{k \in [t+1]} )$
  \vspace{5pt}
\item[] {\it // Disperse encrypted shares}
\item For each $\P_i$:
  \begin{itemize}
  \item[] For $k \in [t+1]$:
      \begin{itemize}
      \item[] $w_{i,k} \leftarrow \msf{PolyWitness}(SP, C_k, \msf{aux}_k, i)$
      \item[] $z_{i,k} \leftarrow \msf{Enc}_{PK_{i}}( \phi(i,k) \| w_{i,k} )$
      \end{itemize}
    \item[] $\msf{AVID}[i].\msf{disperse}(\{ z_{i,k} \}_{k \in [t+1]})$
  \end{itemize}
\end{itemize}
\end{boxedminipage}%
\begin{boxedminipage}{\columnwidth}

{\bf As party $\P_i$:}
\begin{itemize}
\item Wait to receive $\{C_k\}_{k \in [t+1]}$ from $\msf{ReliableBroadcast}$
\item For $j \in [n]$, wait until $\msf{AVID}[j].\msf{disperse}$ completes
  \vspace{5pt}
\item[]  {\it // Decrypt and validate}
\item $\{z_{i,k} \}_{k \in [t+1]} \leftarrow \msf{AVID}[i].\msf{retrieve}()$
\item For $k \in [t+1]$:
  \begin{itemize}
  \item[] $\share{s_k}^{(i)} \| w_{i,k} \leftarrow \msf{Dec}_{SK_i}(z_{i,k})$
  \item[] If $\msf{VerifyEval}(SP, C_k, i, \share{s_k}^{(i)}, w_{i,k}) \neq 1$:
    \begin{itemize}
    \item[] Multicast $(\mtt{IMPLICATE}, \msf{SK}_i, k)$
    \item[] Go to procedure {\bf Share Recovery}
    \end{itemize}
  \end{itemize}
\item Multicast $\mtt{OK}$
\item Wait to receive $\mtt{OK}$ from $2t+1$ different parties
\item Finally \textbf{output} $\{\share{s_k}^{(i)}\}_{k \in [t+1]}$
\end{itemize}

  
{\bf Handle Implication:}
\begin{itemize}
\item on receiving $(\mtt{IMPLICATE}, \msf{SK}_j, k)$ from any $\P_j$:
  \begin{itemize}
  \item[] Discard if $g^{\msf{SK}_j} \neq \msf{PK}_j$
  \item[] $\{ \ldots, z_{j,k}, \ldots \} \leftarrow \msf{AVID}[j].\msf{retrieve}$
  \item[] $\share{s_k}^{(j)} \| w_{j,k} \leftarrow \msf{Dec}_{SK_j}(z_{j,k})$
  \item[] Discard if $\msf{VerifyEval}(SP, C_{k}, j, \share{s_{k}}^{(j)}, w_{j,k}) = 1$
  \item[] Run procedure {\bf Share Recovery}
  \end{itemize}
\end{itemize}

{\bf Share Recovery:}
\begin{itemize}
\item Interpolate $\{C_k\}_{k \in [n]}$ from $\{C_k\}_{k \in [t+1]}$ 
\item If we have previous output shares $\{ \share{s_k}^{(i)} \}_{k \in [t+1]}$,
  \begin{itemize}
  \item[] Interpolate all shares and witnesses $\{ \phi(i, k), w_{i, k} \}_{k \in [n]}$,
  \item[] For each $\P_j$,
    send $(\mtt{R1}, \phi(i, j), w_{i, j})$ to $\P_j$
  \end{itemize}
\item Wait to receive $(\mtt{R1}, \phi(k,i), w_{k, i})$ from $t+1$ different parties, such that ${\msf{VerifyEval}(SP, C_{i}, k, \phi(k, i), w_{k,i}) = 1}$,
  \begin{itemize}
  \item[] Interpolate shares $\phi(\cdot, i)$
  \item[] For each $\P_j$, 
    send $(\mtt{R2}, \phi(j,i), w_{j, i})$ to $\P_j$
  \item[] Wait to receive $(\mtt{R2}, s_{i,k}, w_{i, k})$ from $t+1$ different parties, such that ${\msf{VerifyEval}(SP, C_{k}, i, \phi(i,k)) = 1}$,
  \item[] Interpolate shares $\phi(i, \cdot)$ and {\bf output} $\{ \share{s_k}^{(i)} \}_{k \in [t+1]}$
  \end{itemize}
\end{itemize}
\end{boxedminipage}
\caption{HBAVSS protocol}
\label{alg:hbavss}
\end{figure*}


==> hbavid.tex <==

\subsection{Batch Information Dispersal \textsf{hbAVID} }
In this section we explain a verifiable information dispersal protocol that achieves.

\begin{figure}[t]
\begin{boxedminipage}{\columnwidth}
{\centering \textbf{Algorithm $\msf{hbAVID}(D,R)$ (with Dealer $D$ and Receiver $R$)} \\}
Dispersal
%{ \vspace{1pt} \hline \vspace{1pt} } \\
As dealer $D$:
\begin{itemize}
\item upon input$(v)$:
  \begin{itemize}
  \item[] let $\{s_j\}_{j\in[N]}$ be the blocks of an $(N-2f,N)$-erasure coding scheme applied to $v$
  \item[] let $h$ be a Merkle tree root computed over $\{s_j\}$
  \item[] distribute $h$ via $\msf{ReliableBroadcast}(h)$
  \item[] send $\mtt{VAL}(b_j, s_j)$ to each party $\P_j$, where $b_j$ is the $j^{th}$ Merkle tree branch
  \end{itemize}
\end{itemize}
As party $\P_i$:
\begin{itemize}
\item upon receiving $\mtt{VAL}(b_i, s_i)$ from $D$,
  \begin{itemize}
  \item[] send $\mtt{ECHO}(b_i,s_i)$ to $R$
  \item[] check that $b_i$ is a valid Merkle branch for root $h$ and leaf $s_i$ and if so, multicast $\mtt{OK}$
  \end{itemize}
\end{itemize}
As party $R$:
\begin{itemize}
\item upon receiving $\mtt{ECHO}(b_j,s_j)$ from party $\P_j$, 
  \begin{itemize}
  \item[] check that $b_j$ is a valid Merkle branch for root $h$ and leaf $s_j$, and otherwise discard
  \end{itemize}
\item upon receiving valid $\mtt{ECHO}(\cdot,\cdot)$ messages from $f+1$ distinct parties,
  \begin{itemize}
  \item[] interpolate $\{s_j\}_{j\in[N]}$ from the $f+1$ leaves 
  \item[] recompute Merkle root $h'$ and if $h' \neq h$ then $\mtt{ReliableBroadcast}(\mtt{REVEAL},\{{b_j}, {s_j}\}_{j\in[f+1]})$, where $(b_j, s_j)$ are branch and leaf combinations that verify against $h$
  \item[] otherwise, decode and output $v$
  \end{itemize}
\item if it is later necessary to prove that $v$ was dealt by $D$,
  \begin{itemize}
    \item[] $\mtt{ReliableBroadcast}(\mtt{REVEAL},\{{b_j}, {s_j}\}_{j\in[f+1]})$, where $(b_j, s_j)$ is a valid branch and leaf combination 
  \end{itemize}
\end{itemize}
{\bf Retrieve:}
%{ \vspace{2pt} \hline \vspace{2pt} } \\
\begin{itemize}
\item upon receiving $\mtt{REVEAL}(\{{b_j}, {s_j}\}_{j\in[f+1]})$ from $R$ ,
  \begin{itemize}
  \item[] verify correctness of the branches and leaves against h
  \item[] recalculate the Merkle root as $h'$.
  \item[] wait until $\mtt{OK}$ has been received from $2f+1$ parties
  \item[] If $h \neq h'$, output $\bot$
  \item[] otherwise, decode and output $v$
  \end{itemize}
\end{itemize}
\end{boxedminipage}
\caption{Reliable Point To Point messaging algorithm.}
\label{alg:rp2p}
\end{figure}


==> hbavss-list.tex <==
\begin{figure*}
  \vspace{10pt}
\begin{boxedminipage}{\columnwidth}
  {\centering \textbf{Algorithm $\msf{hbAVSS}(D)$ (for dealer $D$)} \\}
  {\bf Setup:}
\begin{itemize}
\item Each party $P_i$ is associated with a public key $PK_i$, and knows their own secret key $SK_i$ and public generator $g$, such that $PK_i = g^{SK_i}$
\item Setup the polynomial commitment scheme $SP \leftarrow \msf{Setup}(1^\lambda)$
\end{itemize}
{\bf As dealer $D$:} \\
On input $\{s_1,...,s_{t+1}\}$:
\begin{itemize}
\item[] {\it // Secret share encoding}
\item Generate a random degree-$(t,t)$ bivariate polynomial $\phi(\cdot,\cdot)$ so that $\phi(0,k) = s_k$ and $\phi(i,k)$ is $\P_i$'s share of $s_k$
  \vspace{5pt}
\item[] {\it // Broadcast polynomial commitments}
\item For $k \in [t+1]$: $C_k,\msf{aux}_k \leftarrow \msf{PolyCommit}(SP, \phi(\cdot,k) )$
\item $\msf{ReliableBroadcast}( \{ C_k\}_{k \in [t+1]} )$
  \vspace{5pt}
\item[] {\it // Disperse encrypted shares}
\item For each $\P_i$:
  \begin{itemize}
  \item[] For $k \in [t+1]$:
      \begin{itemize}
      \item[] $w_{i,k} \leftarrow \msf{PolyWitness}(SP, C_k, \msf{aux}_k, i)$
      \item[] $z_{i,k} \leftarrow \msf{Enc}_{PK_{i}}( \phi(i,k) \| w_{i,k} )$
      \end{itemize}
    \item[] $\msf{AVID}[i].\msf{disperse}(\{ z_{i,k} \}_{k \in [t+1]})$
  \end{itemize}
\end{itemize}
\end{boxedminipage}%
\begin{boxedminipage}{\columnwidth}

{\bf As party $\P_i$:}
\begin{itemize}
\item Wait to receive $\{C_k\}_{k \in [t+1]}$ from $\msf{ReliableBroadcast}$
\item For $j \in [n]$, wait until $\msf{AVID}[j].\msf{disperse}$ completes
  \vspace{5pt}
\item[]  {\it // Decrypt and validate}
\item $\{z_{i,k} \}_{k \in [t+1]} \leftarrow \msf{AVID}[i].\msf{retrieve}()$
\item For $k \in [t+1]$:
  \begin{itemize}
  \item[] $\share{s_k}^{(i)} \| w_{i,k} \leftarrow \msf{Dec}_{SK_i}(z_{i,k})$
  \item[] If $\msf{VerifyEval}(SP, C_k, i, \share{s_k}^{(i)}, w_{i,k}) \neq 1$:
    \begin{itemize}
    \item[] Multicast $(\mtt{IMPLICATE}, \msf{SK}_i, k)$
    \item[] Go to procedure {\bf Share Recovery}
    \end{itemize}
  \end{itemize}
\item Multicast $\mtt{OK}$
\item Wait to receive $\mtt{OK}$ from $2t+1$ different parties
\item Finally \textbf{output} $\{\share{s_k}^{(i)}\}_{k \in [t+1]}$
\end{itemize}

  
{\bf Handle Implication:}
\begin{itemize}
\item on receiving $(\mtt{IMPLICATE}, \msf{SK}_j, k)$ from any $\P_j$:
  \begin{itemize}
  \item[] Discard if $g^{\msf{SK}_j} \neq \msf{PK}_j$
  \item[] $\{ \ldots, z_{j,k}, \ldots \} \leftarrow \msf{AVID}[j].\msf{retrieve}$
  \item[] $\share{s_k}^{(j)} \| w_{j,k} \leftarrow \msf{Dec}_{SK_j}(z_{j,k})$
  \item[] Discard if $\msf{VerifyEval}(SP, C_{k}, j, \share{s_{k}}^{(j)}, w_{j,k}) = 1$
  \item[] Run procedure {\bf Share Recovery}
  \end{itemize}
\end{itemize}

{\bf Share Recovery:}
\begin{itemize}
\item Interpolate $\{C_k\}_{k \in [n]}$ from $\{C_k\}_{k \in [t+1]}$ 
\item If we have previous output shares $\{ \share{s_k}^{(i)} \}_{k \in [t+1]}$,
  \begin{itemize}
  \item[] Interpolate all shares and witnesses $\{ \phi(i, k), w_{i, k} \}_{k \in [n]}$,
  \item[] For each $\P_j$,
    send $(\mtt{R1}, \phi(i, j), w_{i, j})$ to $\P_j$
  \end{itemize}
\item Wait to receive $(\mtt{R1}, \phi(k,i), w_{k, i})$ from $t+1$ different parties, such that ${\msf{VerifyEval}(SP, C_{i}, k, \phi(k, i), w_{k,i}) = 1}$,
  \begin{itemize}
  \item[] Interpolate shares $\phi(\cdot, i)$
  \item[] For each $\P_j$, 
    send $(\mtt{R2}, \phi(j,i), w_{j, i})$ to $\P_j$
  \item[] Wait to receive $(\mtt{R2}, s_{i,k}, w_{i, k})$ from $t+1$ different parties, such that ${\msf{VerifyEval}(SP, C_{k}, i, \phi(i,k)) = 1}$,
  \item[] Interpolate shares $\phi(i, \cdot)$ and {\bf output} $\{ \share{s_k}^{(i)} \}_{k \in [t+1]}$
  \end{itemize}
\end{itemize}
\end{boxedminipage}
\caption{HBAVSS protocol}
\label{alg:hbavss}
\end{figure*}


==> hbavsslite.tex <==
\section{hbAVSS-Lite}\label{sec:hbavsslite}

We first introduce hbAVSS-Lite, an AVSS protocol that provides linear communication overhead for the dealer with respect to the number of nodes, and which uses simple cryptographic operations to minimize the work that needs to be done by the dealer. Minimizing bandwidth and computation for a resource-constrained dealer is the primary design goal of this protocol.

Previous protocols that achieve fully asynchronous VSS \cite{backes2013asynchronous,cachin2002asynchronous} are based on secet sharing with a bivariate polynomial $f(x,y)$ (with the secret at $f(0,0)$) where participant $P_i$ receives $f(x,i)$, sends $f(j,i)$ to other parties $P_j$, and receives from other parties points to reconstruct $f(i,0)$ which is used as the secret share. In this way, if a party does not receive a message from the dealer, they receive enough information from the other participants to reconstruct their share.
However, this requires the dealer to communicate $O(n^2)$ data. We aim to reduce this requirement while retaining many of the same useful properties of previous schemes.

\begin{figure}
  \vspace{10pt}
\begin{boxedminipage}{\columnwidth}
  {\centering \textbf{Algorithm $\msf{hbAVSS}$-${lite}(D, {\P_i}, s)$} \\}
  Setup:
\begin{itemize}
\item Each party $P_i$ is associated with a public key $PK_i$, and knows their own secret key $SK_i$ and public generator $g$, such that $PK_i = g^{SK_i}$
\item Setup the public parameters: $SP \leftarrow Setup(1^\lambda)$
\end{itemize}
As dealer $D$:
\begin{itemize}
\item on input $s$:
  \begin{itemize}
  \item Sample a random degree-$t$ polynomial $\phi(\cdot)$ with $\phi(0) = s$
  \item Commit to $\phi$: $C,\msf{aux} \leftarrow \msf{PolyCommit}( \phi )$
  \item Sample an ephemeral secret key \(SK_{d}\) and public key \(PK_{d} = g^{SK_{d}}\)
  \item for each $\P_i$:
    \begin{itemize}
    \item $w_i \leftarrow \msf{CreateWitness}(SP, C, \msf{aux}, i)$
    \item Let a shared symmetric key be $ K_{d,i} = PK_{i}^{SK_{d}} $
    \item $z_i \leftarrow \msf{Enc}_{\hash(K_{d,i})}( \phi(i) \| w_i )$
    \end{itemize}
  \item $\msf{ReliableBroadcast}( C \| PK_d \| \{z_i\}_{i \in [n]} )$
  \end{itemize}
\end{itemize}

As party $\P_i$:
\begin{itemize}
\item wait for output $( C \| PK_d \| \{z_i\}_{i \in [n]} )$ from $\msf{ReliableBroadcast}$
  \begin{itemize}
  \item Compute shared key with the dealer \(K_{d,i} = PK_{d,i}^{SK_{i}}\)
  \item $(\share{s}^{(i)} \| w_i) := \msf{Dec}_{\hash(K_{d,i})}(z_i)$
  \item if $\msf{VerifyEval}(SP, C, i, \share{s}^{(i)}, w_i) = 1$:
    \begin{itemize}
    \item multicast $\mtt{OK}$ \anote{the asterisks look bad. also, line numbers would make this easier to refer to}
    \item wait to receive $\mtt{OK}$ from $2t+1$ different parties
    \item \textbf{output} $\share{s}^{(i)}$
    \end{itemize}
  \item else: Let $\pi_i \leftarrow ZK\{(SK_i):g^{SK_i} = PK_i$ and $PK_d^{SK_i} = K_{i,d}\}$
    \begin{itemize}
    \item multicast $(\mtt{IMPLICATE}, {K_{i,d}}, {\pi_i})$
    \item wait to receive $t+1$ $(\mtt{RECOVER}, {\hash (K_{j,d})})$ messages where ${\hash (K_{j,d})}$ decrypts $z_j$ and $\msf{VerifyEval}( SP, C, j, \share{s}^{(j)}, w_j ) = 1$
    \item interpolate $\phi(\cdot)$ and \textbf{output} $\share{s}^{(i)}$
    \end{itemize}
  \end{itemize}

\item on receiving $(\mtt{IMPLICATE}, {K_{j,d}}, {\pi_j})$ from any $\P_j$:
  \begin{itemize}
  \item validate the proof $\pi_j$, counting the message as an \mtt{OK} if validation fails
  \item decrypt share $(\share{s}^{(j)} \| w_j) \leftarrow \msf{Dec}_{\hash(K_{d,j})}(z_j)$
  \item if $\msf{VerifyEval}( SP, C, j, \share{s}^{(j)}, w_j )$ fails:
    \begin{itemize}
      %\item multicast $(\mtt{IMPLICATE}, {K_{i,d}}, {\pi_i})$  (only once)
      \item multicast $(\mtt{RECOVER}, {\hash (K_{i,d})})$  (only once)
    \end{itemize}
  \item else:
    \begin{itemize}
    \item increment the \mtt{OK} message counter if an \mtt{OK} message has not yet been received from $P_j$
    \item if $t+1$ valid shares have been recovered,  interpolate the polynomial $\phi(\cdot)$ and \textbf{output} $\share{s}^{(i)} = \phi(i)$
    \end{itemize}
  \end{itemize}
\end{itemize}

\end{boxedminipage}
\caption{Our hbAVSS-light protocol}
\label{alg:hbavsslight}
\end{figure}


\subsection{Overview of hbAVSS-light}
Our key insight is that we can replace the bivariate polynomial and instead use a univariate polynomial and encryption. In hbAVSS-light, the dealer creates a univariate polynomial and encrypts each share with a different key (which can be derived without prior interaction between the dealer and recipients). Every participant receives and helps disperse the same message, which contains all of the encrypted shares, with each participant being able to decrypt one unique share. At this point the dealer is finished and the receivers decide amongst themselves whether everyone has a valid share. Details about our protocol are given below and the full protocol is presented in Figure~\ref{alg:hbavsslight}.

%The overall flow is that the dealer sends a single round of messages, one to each server. The shares are broadcast through the network, but encryption keeps them secret for each server. The dealer's message also contains authentication information.
%The challenge is ensuring that if any party outputs information, then there will be enough information to do so. We give more detail on the main steps. The detailed protocol is given in Algorithm~\ref{alg:hbavss}.

\subsubsection{The Dealer's Portion}
\paragraph{Sharing and committing}


The secret $s$ is first represented as polynomial $\phi(x)$, where $\phi(0) = s$ and where each party $P_i$ is supposed to receive one share $\phi(i) = \share{s}^{(i)}$.
  
We use PolyCommitPed-SC (Figure ~\ref{polycommit}) to commit to polynomials in this scheme. $Commit( \phi(x) )$ outputs a commitment $C$, which needs to be sent to all participants. The $CreateWitness$ function creates a data point $w_i$, which when used along with a share in the function $VerifyEval$ allows a recipient to verify that their share is a part of the polynomial committed to by $C$.
\paragraph{Encryption}


In this scheme, the dealer sends the same message to every participant. To ensure the secrecy of shares we rely on hybrid encryption. We assume that every recipient possesses a secret key $SK$ and corresponding public key $PK = g^{SK}$ where $g$ is a public generator of a cyclic group and is used for all public keys. We also assume that there exists a PKI where every server's public key can be found. The dealer creates a one-time keypair, for which the public key will be broadcasted. To encrypt party $P_i$'s share, the dealer $P_d$ looks up the public key $PK_i$ and calculates a symmetric key $K^d_i = PK_i^{SK_d}$, which can also be calculated by $P_i$, and encrypts the share with $\hash(K^d_i)$. This specific construction is chosen to allow parties to share their symmetric key (and prove that it is correctly calculated) without revealing their secret key.
  
\paragraph{ReliableBroadcast}
To amortize the overall bandwidth of our scheme, we utilize the ReliableBroadcast protocol of Cachin and Tessaro, which is reproduced in Figure \ref{alg:rbc}. This protocol allows the dealer to send reliably send the same message to all n participants at a total cost of $\frac{n}{t+1}$ times the size of the broadcasted message plus $n \log n$ hashes for authentication. The end result of the broadcast is a guarantee that all honest participants will agree on the contents of the broadcasted message.

\subsubsection{The Recipients' Portion}
\paragraph{Share Verification}
  After the ReliableBroadcast, each party $P_i$ attempts to decrypt their corresponding share and witness. If decryption is successful and $VerifyEval$ returns \textit{True}, then $P_i$ will relay an \mtt{OK} message.%
% \footnote{This additional round can be suppressed by modifying ReliableBroadcast, as we discuss in the Appendix \anote{TODO}, but for simplicity we keep the existing interface).}
%  Once enough peers $(2t+1)$ report \mtt{OK}, it is safe to use $\share{s}$ in further calculations.

\paragraph{Handling a faulty dealer}

Handling the case of a faulty dealer is the trickiest part of the protocol. Because we are not using a bivariate polynomial, if $P_i$'s correct share is never sent by the dealer, it can not be recovered without reconstructing $\phi(x)$ unless additional information is used. However, we argue that the privacy of a malicious dealer's secret is not worth being concerned about and that it is acceptable to reveal it in a recovery phase if there is definitive proof of a dealer's malfeasance.

The polynomial commitment $C$ is included in the message sent by ReliableBroadcast, so all honest parties must agree on it. Due to the\textit{ Evaluation Binding} property of PolyCommit schemes, it is computationally infeasible for a dealer to generate a $C$ and a witness such that $VerifyEval$ evaluates to \textit{True} for $\share{s}$ if $\share{s}$ is not a share of $s$.

%The secret shares are directly checked against $C$ prior to concluding the protocol, hence if all honest parties output secret shares $\share{s}$, then $\share{s}$ is guaranteed to be a correct $t$-sharing.

  Since each node waits for ReliableBroadcast to terminate before proceeding, if any party outputs a share $\share{s}$, then every party $\P_j$ receives the polynomial commitment $C$ as well as every party's encrypted materials. If $P_i$ is dealt a share that either fails to decrypt or fails verification, they send the message (\mtt{IMPLICATE}, ${K_d}^i$, $\pi$) to all other participants, where $\pi$ is a Non-Interactive Zero Knowledge Proof that the shared key is correct: $ZK\{(SK_i):g^{SK_i} = PK_i$ and $PK_d^{SK_i} = K_{i,d}\}$ \cite{chaum1992wallet}. Upon validating that the implicate message is correct, other parties will begin sharing their own shared keys so that $P_i$ can reconstruct $\share{s}^{(i)}$.
  
\subsection{Security and Property Analysis}
\begin{theorem}
HBAVSS-lite is an AVSS protocol that satisfies Definition \ref{def:avss} as long as all of the following are used in its construction:
\begin{itemize}
  \item A PolyCommit scheme that satisfies Definition \ref{def:polycommit}
  \item A ReliableBroadcast scheme that satisfies Definition \ref{def:rbc}
  \item A correct symmetric encryption scheme that achieves semantic security
  \item A cryptosystem in which the Computational Diffie-Hellman problem is intractable
  \item A reliable Public Key Infrastructure which allows all participants to know the correct public keys of all other participants
\end{itemize}
\end{theorem}
\bigskip

We will now show that hbAVSS-lite meets the \textit{liveness}, \textit{secrecy}, and \textit{agreement} properties required for an AVSS scheme.

\paragraph{Liveness} If the dealer is honest, then all honest participants output a share $\share{s}$.

When the dealer is honest, the broadcasted message contains correctly formatted encrypted shares for all participants. The shared keys are computable due to the assumption of a PKI and the use of a correct symmetric encryption scheme ensures that the shares will be decryptable. 

The \textit{validity} property of ReliableBroadcast guarantees that all honest participants will both receive and agree on this message, even in the presence of $t$ adversarial nodes who can behave arbitrarily. All honest participants will then broadcast $\mtt{OK}$ messages and upon receiving $2t+1$ of them will output $\share{s}$, satisfying \textit{liveness}. This is guaranteed to occur, due to our assumption that our asynchronous network will eventually deliver all messages.

\paragraph{Secrecy} If the dealer is honest, then the adversary does not learn any information about $\share{s}$

As hbAVSS-lite uses Shamir Sharing, for an adversary that controls $t$ recipients to learn information about $s$, they would need to recover information about an additional share. Since the shares that are delivered with ReliableBroadcast are encrypted, to learn about them an adversary would need to backdoor the Setup process or solve the Computational Diffie-Hellman Problem to derive a shared key or be able to break the semantic security of the symmetric encryption scheme. Further, as the polynomial commitment provides unconditional hiding, it does not divulge any information about the polynomial, and thus the secret, to an adversary.

The other option is for an adversary to convince an honest recipient to divulge their share via a false $\mtt{IMPLICATE}$ message. To do so would require the adversary to break the zero-knowledgeness of the Chaum-Pedersen proofs \anote{Where are chaum-pedersen mentioned}, which is avoided due to the choice of an appropriate cryptosystem.

\todo{Should replay attacks still be mentioned somewhere? If so, where and how?} \anote{is it necessary for this proof to be correct?}

\paragraph{Agreement} If any honest party outputs a share $\share{\cdot}$, then there exists a unique value $s$ such that all honest parties output $\share{s}$.

Agreement in the case of an honest dealer follows from \textit{liveness}. As there is no output path which skips ReliableBroadcast, honest participants are guaranteed to receive valid shares of the the same $s$ from an honest dealer. Further, a dishonest dealer can not cause disagreement among honest nodes about the contents of the broadcasted message per the \textit{totality} property of ReliableBroadcast.


The only remaining option is for a malicious dealer to send messages which may not decrypt or may correspond to invalid shares. Since all honest recipients agree on $C$, as per ReliableBroadcast, and the \textit{Evaluation Binding} property of PolyCommit guarantees that $VerifyEval$ returning \textit{True} implies that a share is valid, no honest party with an invalid share will output $\share{s}$. If an honest party outputs $\share{s}$, then it must have received $2t+1$ $\mtt{OK}$ messages, implying that $t+1$ valid shares exist, which means that $s$ is recoverable and that all honest nodes agree on it.

\subsection{Cost Analysis}
\subsubsection{Communication Costs}
\paragraph{Dealer Communication Costs}
The only bandwidth costs faced by the dealer in hbAVSS-lite are those associated with ReliableBroadcast, which for the dealer will be entirely outgoing traffic. The ReliableBroadcast scheme used in this work uses erasure coding to minimize bandwidth and realize an asymptotic bandwidth cost of $O(N\kappa + N\log N)$, where $\kappa$ is the size of the broadcasted message. Specifically, each broadcast recipient expects to receive a size $\frac{\kappa}{N-2t}$ erasure-coded share and a Merkle tree branch consisting of $\ceil{\log_2 (N)}$ hash function outputs. This means that ReliableBrodcast imparts a total outgoing bandwidth cost of $\frac{N}{N-2t} \cdot \kappa + \ceil{\log_2 (N)}h$, where $h$ is the size of a hash function output.

The message that the dealer must broadcast consists of an ephemeral public key, a linear-sized polynomial commitment, and a linear number of encrypted shares and witnesses. We assume that hbAVSS-lite will be best implemented in an elliptic curve cryptosystem, in which case the polynomial commitment and ephemeral key will consist of elliptic curve points, while the shares and witnesses will be integers in a finite field. If we represent elliptic curve points by $c$ and field integers by $f$, then the total bandwidth that needs to be sent by the dealer is represented by $\frac{N}{N-2t} \cdot ((t+2)c + 2Nf) + N\ceil{\log_2 (N)}h$.

\paragraph{Recipient Communication Costs}
In hbAVSS-lite a recipient needs to receive the broadcasted message from the dealer, verify its integrity, and help to recover the secret if the dealer has sent a malformed message. In the best case scenario, besides sending and receiving up to $N$ \mtt{OK} of negligible size, all of the recipient's bandwidth again comes from ReliableBroadcast. A recipient will receive one erasure-coded share from the dealer and $N-1$ shares from other participants, while itself forwarding its share to the other $N-1$ participants. For conciseness, we will round up and state that each participant sends and receives $N$ erasure-coded shares, along with $N$ Merkle branches. The sent and received bandwidth for each recipient then both end up being the same as the dealer's send bandwidth: $\frac{N}{N-2t} \cdot ((t+2)c + 2Nf) + N\ceil{\log_2 (N)}h$.

In the case of a malicious dealer, an additional cost for share reconstruction is incurred. This cost is greatest for a recipient with an invalid share who needs to initiate the implication process. Such a recipient would need to multicast their shared key with the dealer as well as a proof that the key is correct. In this construction, we use a Chaum-Pedersen proof which consists of two elliptic curve points and a field integer. Upon receiving a valid $\mtt{IMPLICATE}$ message, peers will multicast a hash of their shared key with the dealer. 

In an absolute worst case scenario, $2t$ of the recipients will send $\mtt{IMPLICATE}$ messages before receiving any $\mtt{IMPLICATE}$ messages themselves. The worst case receiver in this case will then send $(N-1)\cdot(3c + f)$ and receive $(t+1)h + (2t-1)\cdot(3c + f)$ in addition to the best case costs. Even in this scenario, we note that the asymptotic bandwidth complexity for the recipients has not worsened, though the number of curve points that need to be sent and received increase by a factor of about 4 and 3 respectively.

One could also consider the case of malicious recipients trying to waste the bandwidth of their peers. To do so, all $t$ adversarial nodes could multicast an invalid $\mtt{IMPLICATE}$ message, causing every honest node to receive an additional $t\cdot(3c + f)$. Of course, doing so will clearly reveal malicious intent and should be considered comparable to trying to DOS the network with arbitrary traffic. We consider the problem of handling provably malicious peers out of scope for this work.

\subsubsection{Computation Costs}
\paragraph{Dealer Computation Costs}
hbAVSS-lite is designed to minimize the work of the dealer. Computationally, this is done by using a version of PolyCommitPed with simplified cryptography, which we call PolyCommitPed-SC. One of the most significant costs of PolyCommitPed is that of witness creation. A dealer needs to create witnesses to accompany every share it creates, which for PolyCommitPed involves multiple elliptic curve scalar multiplications. In contrast, witnesses in PolyCommitPed-SC are created using only operations on finite field elements, resulting in greatly improved performance. 

The total computational work that needs to be done by an hbAVSS-lite dealer is as follows:
\begin{itemize}
    \item Sample a degree-$t$ sharing polynomial $\phi(\cdot)$. This only involves sampling $t+1$ random field integers and is negligible.
    \item Commit to $\phi(\cdot)$. This involves randomly sampling a hiding polynomial $\hat{\phi}(\cdot)$ and using it to make Pedersen commitments to the coefficients of $\phi(\cdot)$ using public curve points $g$ and $h$. This only requires $2t + 2$ curve point scalar multiplications (tables for which can be precomputed) and $t$ curve point additions.
    \item Create shares and witnesses for each recipient. This can be done by solving $2$ degree-$t$ polynomials for $N$ points each. Using Horner's rule, this only requires $2N(t+1)$ field additions and $2Nt$ field multiplications.
    \item Generate shared keys with recipients. This involves $N$ curve point scalar multiplications (tables can also be precomputed here) and $N$ hashes (negligible).
    \item Encrypt the messages and send them using ReliableBroadcast. The computational work here is only performing $N$ symmetric encryptions, erasure-coding the message, and taking $N\log N$ hashes, all of which are incredibly quick on modern devices.
\end{itemize}
In all, the dealer is primarily concerned with performing a linear number of elliptic curve operations and a quadratic number of finite field operations leading to a very low overall computational cost.



==> model.tex <==
\section{Problem Definition And Solution Overview}
\subsection{System Model}
For this work, we consider an asynchronous network model. We assume that any node in the network can send a message to any other node, but that this message may be delayed for an arbitrary and unbounded amount of time. In addition, a global adversary is able to monitor all messages sent over the network, delay them for an arbitrary amount of time, and deliver them out of order but can not modify them or prevent them from being sent indefinitely. To that end, we consider that any timeout in the protocol will always occur and that timeouts are best avoided.

We assume that for any protocol or subprotocol used in this work, up to $t$ nodes are controlled by a Byzantine adversary (who can also collude with the global adversary), such that $t < \frac{N}{3}$, where $N$ is the total number of nodes participating in the protocol. These Byzantine adversaries can fail to respond to messages, craft and send malicious messages, and collude with each other to coordinate attacks. We do not consider Sybil attacks, which could otherwise allow an attacker to gain control of a byzantine quorum of the network. These should be addressed by an architect who uses our protocols in their own system. Similarly, although our Byzantine adversaries can send invalid messages to try to thwart the protocols, we consider the problem of an adversary trying to DOS the network by sending very large amounts of invalid data to be out of scope.

We further assume the existence of an available and accurate public key infrastructure, which nodes can use to learn the public keys of other nodes in the network. Lastly, we assume that if two honest parties wish to communicate with each other, the receiver can determine whether or not a particular message came from a sender. 

\subsection{Asynchronous Verifiable Secret Sharing}
\begin{definition}(Asynchronous Verifiable Secret Sharing (AVSS))
  Consider a dealer $D$ and $N > 3t$ parties, where we assume an adversary may corrupt up to $t$ of the parties and possibly the dealer. 
  In an AVSS protocol, the dealer receives input $s \in \field$, and each party $P_i$ may receive an output share $\share{s}^{(i)}$. The protocol must satisfy the following properties:
\begin{itemize}
\item \emph{(Liveness)}: If the dealer $D$ is honest, then all honest parties eventually output a share \share{s}.
\item \emph{(Secrecy)}: If the dealer $D$ is honest, then the adversary does not learn any information about $s$
\item \emph{(Agreement)}: If any honest party outputs a share $\share{\cdot}$, then there exists a unique value $s$ such that all honest parties output $\share{s}$.
\end{itemize}
\label{def:avss}
\end{definition}

Our liveness property implies that as long as the dealer is honest and no more than $t$ nodes are corrupted, then honest nodes are guaranteed output. In Feldman's original verifiable secret sharing protocol, an adversary that corrupts even one node may prevent the protocol from outputting a value.

This agreement property is also written carefully to incorporate the \emph{strong commitment} property due to Backes et al.~\cite{eavss}, in which the unique agreed-upon value $s$ is already determined at the time that the first honest party outputs a share (and cannot be influenced thereafter by the adversary).

\subsection{System Goals}

\begin{description}
\item[Fully Asynchronous:] We aim for our protocols to operate as quickly as the network will allow, regardless of the quality of said network, and with no parameter tuning required. To that end, it is imperative that our protocol's performance is not negatively impacted by slow messages. To accomplish this, we eschew the use of timeouts in any of our protocols.
\item[Optimally Byzantine Fault Tolerant:] We envision that our protocol may be deployed in a decentralized system in which there is no mutual trust between nodes, such as a permissionless blockchain. Participants in such a setting may have a motivation, economic or otherwise, to corrupt the protocol and collusion should be tolerated to an optimal degree. This also ties in with asynchrony, in that assuming that a node has crashed because it does not appear to have sent a message within a specified timeframe could potentially result in an honest node being removed from the network, thus degrading security.
\item[Scalable:] We aim for protocols which obtain not only good asymptotic communication and computation complexities, but do so with low constant factors. Our two AVSS protocols, hbAVSS-lite and hbAVSS, minimize the dealer's overhead and the overall protocol overhead respectively.
\end{description}

\subsection{Solution Overview}
Our AVSS protocols make use of efficient reliable asynchronous messaging primitives in order to facilitate fault-tolerant delivery of secret shares. Since using such protocols exposes message contents to protocol participants, we add in a layer of encryption to safeguard this information. Lastly, to facilitate share recovery in the presence of faults, we design a mechanism to allow recipients to prove whether a dealer has sent a malformed message, and if so, initiate reconstruction.

In hbAVSS-lite, we optimize for the dealer's computation and communication overhead by using simpler cryptographic operations and sending all encrypted shares in one efficiently-broadcasted message. hbAVSS uses an additional primitive, \todo{rp2p new name}, to send each recipient their encrypted share while still allowing for the dealer to be implicated of malfeasance. This allows for an asymptotic bandwidth improvement to the overall protocol.

Using these primitives allows us to achieve robust, asynchronous secret sharing while only using a univariate polynomial. This is in contrast to previous optimally fault-tolerant AVSS constructions such as \todo{cite} which relied on multivariate polynomials and saw nonlinear asymptotic overheads as a result. In contrast to the concurrent work of Rasu et al \todo{cite}, which also uses a univariate polynomial, our protocols do not rely on timeouts or on any particular connection being fast, resulting in asymptotically better performance in non-optimal scenarios. A fuller comparison with other AVSS approaches is given in section \todo{ref}.

==> rbc.tex <==
\subsection{Communication-optimal reliable broadcast.}
Broadcast algorithms are a crucial component of many verifiable secret sharing schemes. Particularly, it may be necessary to use a \textit{reliable broadcast} in which all honest participants in a protocol agree on the same broadcasted value. 
\begin{definition} (Reliable Broadcast)
Consider a dealer $D$ and $N > 3t$ parties, where we assume an adversary may corrupt up to $t$ of the parties and possibly the dealer. A Reliable Broadcast protocol will achieve the following properties:
\begin{itemize}
  \item \emph{(Agreement)} If any two correct nodes deliver $v$ and $v'$, then $v = v'$.
  \item \emph{(Totality)} If any correct node delivers $v$, then all correct nodes deliver $v$
  \item \emph{(Validity)} If the sender is correct and inputs $v$, then all correct nodes deliver $v$
\end{itemize}
\label{def:rbc}
\end{definition}

While Bracha's~\cite{bra87} classic reliable broadcast protocol requires $O(N^2|v|)$ bits of total communication in order to broadcast a message of size $|v|$, Cachin and Tessaro~\cite{dispersal} observed that erasure coding and hash trees can be used to reduce this cost to merely $O(N|v| + \lambda N^2 \log N)$, even in the worst case. Since the nonlinear component of this complexity is not dependent on the size of the message being sent, if a sufficiently large batch of messages is sent at once, the cost per message is linear.

If the sender is correct, the total running time is three (asynchronous) rounds; and in any case, at most two rounds elapse between when the first correct node outputs a value and the last outputs a value. The reliable broadcast algorithm of Cachin and Tessaro is shown in Figure~\ref{alg:rbc}.

\begin{figure}[t]
\begin{boxedminipage}{\columnwidth}
{\centering \textbf{Algorithm $\msf{RBC}(D)$ (with Dealer $D$)} \\}
As dealer $D$:
\begin{itemize}
\item upon input$(v)$:
  \begin{itemize}
  \item[] let $\{s_j\}_{j\in[N]}$ be the blocks of an $(N-2f,N)$-erasure coding scheme applied to $v$
  \item[] let $h$ be a Merkle tree root computed over $\{s_j\}$
  \item[] send $\mtt{VAL}(h, b_j, s_j)$ to each party $\P_j$, where $b_j$ is the $j^{th}$ Merkle tree branch
  \end{itemize}
\end{itemize}
As party $\P_i$:
\begin{itemize}
\item upon receiving $\mtt{VAL}(h, b_i, s_i)$ from $\P_\msf{Sender}$,
  \begin{itemize}
  \item[] multicast $\mtt{ECHO}(h,b_i,s_i)$
  \end{itemize} 
\item upon receiving $\mtt{ECHO}(h,b_j,s_j)$ from party $\P_j$, 
  \begin{itemize}
  \item[] check that $b_j$ is a valid Merkle branch for root $h$ and leaf $s_j$, and otherwise discard
  \end{itemize}
\item upon receiving valid $\mtt{ECHO}(h,\cdot,\cdot)$ messages from $N-f$ distinct parties,
  \begin{itemize}
  \item interpolate $\{s'_j\}$ from any $N-2f$ leaves received
  \item recompute Merkle root $h'$ and if $h' \neq h$ then abort        \item if $\mtt{READY}(h)$ has not yet been sent, multicast $\mtt{READY}(h)$
  \end{itemize}
\item upon receiving $f+1$ matching $\mtt{READY}(h)$ messages, if $\mtt{READY}$ has not yet been sent, multicast $\mtt{READY}(h)$
\item upon receiving $2f+1$ matching $\mtt{READY}(h)$ messages, wait for $N-2f$ \mtt{ECHO} messages, then decode $v$
\end{itemize}
\end{boxedminipage}
\caption{Reliable broadcast algorithm from Cachin and Tessaro~\cite{dispersal}, which combines Bracha broadcast~\cite{bra87} with erasure codes to improve efficiency.}
\label{alg:rbc}
\end{figure}

